Advances in Observing Various Coronal EUV Waves in the SDO Era and Their Seismological Applications (Invited Review)

Global extreme ultraviolet (EUV) waves are spectacular traveling disturbances in the solar corona associated with energetic eruptions such as coronal mass ejections (CMEs) and flares. Over the past 15 years, observations from three generations of space-borne EUV telescopes have shaped our understanding of this phenomenon and at the same time led to controversy about its physical nature. Since its launch in 2010, the Atmospheric Imaging Assembly (AIA) onboard the Solar Dynamics Observatory (SDO) has observed more than 210 global EUV waves in exquisite detail, thanks to its high spatio-temporal resolution and full-disk, wide-temperature coverage. A combination of statistical analysis of this large sample, 30 some detailed case studies, and data-driven MHD modeling, has been leading their physical interpretations to a convergence, favoring a bimodal composition of an outer, fast-mode magnetosonic wave component and an inner, non-wave CME component. Adding to this multifaceted picture, AIA has also discovered new EUV wave and wave-like phenomena associated with various eruptions, including quasi-periodic fast propagating (QFP) wave trains, magnetic Kelvin-Helmholtz instabilities (KHI) in the corona and associated nonlinear waves, and a variety of mini EUV waves. Seismological applications using such waves are now being actively pursued, especially for the global corona. We review such advances in EUV wave research focusing on recent SDO/AIA observations, their seismological applications, related data analysis techniques, and numerical and analytical models.

==> abstract.tex <==

\title{Advances in Observing Various Coronal EUV Waves in the SDO Era and Their Seismological Applications (Invited Review)}

\author{Wei Liu
        Leon Ofman
       }

\runningauthor{Liu \& Ofman}
\runningtitle{EUV Wave Observations by SDO/AIA}


\institute{
 W.~W.~Hansen Experimental Physics Laboratory, Stanford University, Stanford, CA 94305, USA; Lockheed Martin Solar and Astrophysics Laboratory, Bldg.~252, 3251 Hanover Street, Palo Alto, CA 94304, USA
   email: \url{weiliu@lmsal.com} 
 Catholic University of America and NASA Goddard Space Flight Center, Code 671, Greenbelt, MD 20771, USA; Visiting Associate Professor, Department of Geophysics and Planetary Sciences, Tel Aviv University, Tel Aviv 69978, Israel
   email: \url{Leon.Ofman@nasa.gov}
}


\begin{abstract}	

Global extreme ultraviolet (EUV) waves are spectacular traveling disturbances in the solar corona associated with energetic eruptions such as coronal mass ejections (CMEs) and flares. Over the past 15 years, observations from three generations of space-borne EUV telescopes have shaped our understanding of this phenomenon and at the same time led to controversy about its physical nature. Since its launch in 2010, the Atmospheric Imaging Assembly (AIA) onboard the Solar Dynamics Observatory (SDO) has observed more than 210 global EUV waves in exquisite detail, thanks to its high spatio-temporal resolution and full-disk, wide-temperature coverage. A combination of statistical analysis of this large sample, 30 some detailed case studies, and data-driven MHD modeling, has been leading their physical interpretations to a convergence, favoring a bimodal composition of an outer, fast-mode magnetosonic wave component and an inner, non-wave CME component. Adding to this multifaceted picture, AIA has also discovered new EUV wave and wave-like phenomena associated with various eruptions, including quasi-periodic fast propagating (QFP) wave trains, magnetic Kelvin-Helmholtz instabilities (KHI) in the corona and associated nonlinear waves, and a variety of mini EUV waves. Seismological applications using such waves are now being actively pursued, especially for the global corona. We review such advances in EUV wave research focusing on recent SDO/AIA observations, their seismological applications, related data analysis techniques, and numerical and analytical models.

\end{abstract}

\keywords{Corona, Structures; Coronal Mass Ejections, Low Coronal Signatures; Coronal Seismology; Flares, Waves; 
Waves, magnetohydrodynamic; Waves, propagation}


--- figs and other files ---------------
1) submit as "Figure" (will unzip online)

 zip figs.zip f*.*

2) submit as "attachment to manuscript"
 zip ms_attachment.zip ms.bbl_edit *.sty
  adding: ms.bbl_edit (deflated 82%)
  adding: solar_physics_additional_label_def.sty (deflated 66%)
  adding: style_wei.sty (deflated 61%)
  adding: style_wei_symbols.sty (deflated 71%)


--- comments -------------------
(1) Somehow in the generated PDF, Figure 11 left panels and Figure 16 right panel do not appear in the right portion, although they are fine in my locally generated ms.pdf file. In both cases, I use the bb option in  \includegraphics to specify the desired portion of a large .eps file to be displayed, i.e.,

\includegraphics[height=5.1cm, bb=117 195 334 675, clip]{fig_Yuan_2013AA_f1_orig.eps}
\includegraphics[height=3.8cm, bb=73 36 195 161, clip]{fig_Pascoe_2013AA_f5a_w-axes_res300.eps}

(2) Tables 5 and 6 have overflow on the right hand side, although they are fine in my locally generated ms.pdf file.

